A deep learning based tool for automatic brain extraction from functional magnetic resonance images in rodents

Removing skull artifacts from functional magnetic images (fMRI) is a well understood and frequently encountered problem. Because the fMRI field has grown mostly due to human studies, many new tools were developed to handle human data. Nonetheless, these tools are not equally useful to handle the data derived from animal studies, especially from rodents. This represents a major problem to the field because rodent studies generate larger datasets from larger populations, which implies that preprocessing these images manually to remove the skull becomes a bottleneck in the data analysis pipeline. In this study, we address this problem by implementing a neural network based method that uses a U-Net architecture to segment the brain area into a mask and removing the skull and other tissues from the image. We demonstrate several strategies to speed up the process of generating the training dataset using watershedding and several strategies for data augmentation that allowed to train faster the U-Net to perform the segmentation. Finally, we deployed the trained network freely available.

==> draft.tex <==
However, rodents can provide robust models for both understanding and diagnosing human psychiatric disorders (Neumann et al., 2011, ++)\cite{dirnberger2015nefi}, and  extensive knowledge about fundamental brain mechanisms have been acquired in rodents using tools that are currently unavailable for use in humans.
The application of fMRI to rodent models has opened up the door to understand the neurobiological underpinnings of the functional networks observed with fMRI, by linking the extensive base of knowledge acquired from rodent neuroscience research to humans.


It  has  been  shown  that several  factors  affect  the  outcome  of  methods  devised  for  removing non-brain tissue. These include imaging artifacts, different MRI scanners and protocols that in turn  lead  to contrast  and  intensity variations.  Further,  anatomical variability, as  well  as  age and  the extent  of brain atrophy, e.g. due  to neurodegeneration, have  been  reported as influencing the results  of  current  brain  extraction  methods (Fennema-Notestine  et  al.,  2006).

This is due to the lower 

However, because the 
this does not work for 

and are therefore commonly carried out by hand. 

, thus improving the data quality. Brain extraction is therefore commonly carried out both on the anatomical images as well as the functional images. A further benefit of extracting the brain in the functional data set is that it improves the quality and speeds up the analysis process. as well as for improving and to remove non-brains signal from the subsequent analysis of the data

. removal of the a step which is necessary both for correct realignment


and with the rapid advancements in field strengths and preclinical scanner accessories the application of fMRI analysis to rodents is a promising tool/method for bridging the gap between the MRI-derived understanding of the human brain and the significantly larger body of knowledge about basic mammalian brain mechanisms in rodents.
 



 based on rodent study, 

holds the promise of bridging the gap between what we know about the mammalian brain from rodent-derived studies using electrophysiology and optical methods While preclinical rodent scanners have also been utilized, the small scale of the rodent brain has meant that However, increasing scanner strenghts as well as a proliferation of supplementary tools accessories that enable the study of smaller mammals during awake trials holds promise for bridging the gap between the large body of knowledge generated by studying the single-cell/population activites of brain cells and the whole-brain activity of rodents. 

possibility of awake imaging in the improvements in hardware and availability of preclinical scanners for studying smaller animals fMRI in small-scale animals have increased over the years, Enabling the investigation Rodent fMRI is
Automation is an important tool for handeling and processing 





There is, to the best of our knowledge, only one related work that presents a method to Skull from....
Find similar work deep learning and skull removal.
In  this  study  we  compare the  proposed method  to six popular  algorithms  that  are  freely available and  commonly  used  for  comparison (Galdames  et  al.,  2012;  Iglesias  et  al.,  2011; Wang et al., 2014).The Brain Extraction Tool1(BET) is a fast and versatile method that uses a deformable model(Smith, 2002). Intensity  and  shape  variations  related  to  tumor presence  might hinder the evolution of the mesh(Speier et al., 2011). Nevertheless,BET performs quite well on these kinds of images.


